E-unification for Second-Order Abstract Syntax

Higher-order unification (HOU) concerns unification of (extensions of) $\lambda$-calculus and can be seen as an instance of equational unification ($E$-unification) modulo $\beta\eta$-equivalence of $\lambda$-terms. We study equational unification of terms in languages with arbitrary variable binding constructions modulo arbitrary second-order equational theories. Abstract syntax with general variable binding and parametrised metavariables allows us to work with arbitrary binders without committing to $\lambda$-calculus or use inconvenient and error-prone term encodings, leading to a more flexible framework. In this paper, we introduce $E$-unification for second-order abstract syntax and describe a unification procedure for such problems, merging ideas from both full HOU and general $E$-unification. We prove that the procedure is sound and complete.

==> figures/metavariable-substitution.tex <==
\begin{figure}
  \begin{mdframed}
  \begin{align*}
    \Theta = (\metavar{M}{_i} : [\type{\overline{\sigma_i}}]\type{\tau_i})^{i \in \{1,\ldots,n\}}
    \quad\quad
    \Theta \mid \Gamma \vdash t : \type{\tau}
    \quad\quad
    \text{for all $i \in \{1, \ldots, n\}$} \; \Xi \mid \Gamma \vdash t_i : \type{\beta_i}\span \\
    t[\metavar{M}{_i}]^{i \in \{1, \ldots, n\}} \; \text{is defined recursively}
    \span \\
    x[\m[\overline{z}] \mapsto t]
    &= x \\
    \m[\overline{s}][\m[\overline{z}] \mapsto t] 
    &= t[\overline{z} \mapsto \overline{s}]
    \quad \text{when $|\overline{s}| = |\overline{z}|$} \\
    \metavar{N}{}[\overline{s}][\m[\overline{z}] \mapsto t]
    &= \metavar{N}{}[s_1, \ldots, s_k]
    \quad \text{when $\metavar{N}{} \not= \m$} \notag \\
    \defcon(\overline{\overline{x}.s})[\m[\overline{z}] \mapsto t]
    &= \defcon(\overline{\overline{x}.s[\m[\overline{z}] \mapsto t]})
  \end{align*}
  \end{mdframed}
  \caption{Metavariable substitution.}
  \label{figure:metavariable-substitution}
\end{figure}


==> figures/procedure-example.tex <==
\begin{figure}
  \begin{mdframed}

  \tiny
  \begin{tikzcd}
    \{
      \highlight{\forall g, y. \con{app}(\metavar{m}{}[], \con{pair}(g, \con{abs}(h.\con{app}(h, y)))) \meq \con{app}(g, y)}
    \}
    \arrow[d,
      "\metasubst{\mathsf{id}}"',
      "\text{\textbf{mutate} via $\con{app}(\con{abs}(x. \metavar{m}{_1}[x,g,y]), \metavar{n}{_1}[g,y]) \equiv \metavar{m}{_1}[\metavar{n}{_1}[g,y],g,y]$}"]
    \\
    \arrow[d,
      "\metasubst{\mathsf{id}}"',
      "\text{\textbf{decompose}}"]
    \\
    %\{ \highlight{\metavar{m}{}[] \meq \con{abs}(x.\metavar{m}{_1}[x])}, \quad
    %   \con{pair}(g, \con{abs}(h.\con{app}(h, y))) \meq \metavar{n}{_1}[], \quad
    % \metavar{m}{_1}[\metavar{n}{_1}[]] \meq \con{app}(g, y) \}
    \arrow[d,
      "\text{$[\metavar{m}{}[] \mapsto \con{abs}(x.\metavar{m}{_2}[x])]$}"',
      "\text{\textbf{imitate}}"]
    \\
    \arrow[d,
      "\text{$[\metavar{m}{_1}[x, g, y] \mapsto \metavar{m}{_2}[x])]$}"',
      "\text{\textbf{eliminate*}}"]
    \\
     %\{ \highlight{\con{pair}(g, \con{abs}(h.\con{app}(h, y))) \meq \metavar{n}{_1}[]}, \quad
    %   \metavar{m}{_2}[\metavar{n}{_1}[]] \meq \con{app}(g, y) \}
    \arrow[d,
      "\text{$[\metavar{n}{_1}[g,y] \mapsto \con{pair}(g, \con{abs}(h.\con{app}(h, y)))]$}"',
      "\text{\textbf{eliminate*}}"]
    \\
    \{
      \highlight{\forall g,y. \metavar{m}{_2}[\con{pair}(g, \con{abs}(h.\con{app}(h, y)))] \meq \con{app}(g, y)}
    \}
    \arrow[d,
      "\text{$[\metavar{m}{_2}[z] \mapsto \con{app}(\metavar{m}{_3}[z], \metavar{m}{_4}[z])]$}"',
      "\text{\textbf{imitate axiom} ($\beta_\lambda$)}"]
    \\
    \arrow[d,
      "\metasubst{\mathsf{id}}"',
      "\text{\textbf{mutate} via $\con{app}(\con{abs}(x. \metavar{m}{_5}[x,g,y]), \metavar{n}{_5}[g,y]) \equiv \metavar{m}{_5}[\metavar{n}{_5}[g,y],g,y]$}"]
    \\
    \arrow[d,
      "\metasubst{\mathsf{id}}"',
      "\text{\textbf{decompose}}"]
    \\
    \arrow[d,
      "\text{$[\metavar{n}{_5}[g,y] \mapsto \metavar{m}{_4}[\con{pair}(g, \con{abs}(h.\con{app}(h, y)))] ]$}"',
      "\text{\textbf{eliminate*}}"]
    \\
    \{
      \highlight{\metavar{m}{_3}[\con{pair}(g, \con{abs}(h.\con{app}(h, y)))] \meq \con{abs}(x.\metavar{m}{_5}[x,g,y])},
      \metavar{m}{_5}[\metavar{m}{_4}[\con{pair}(g, \con{abs}(h.\con{app}(h, y)))],g,y] \meq \con{app}(g, y)
    \}
    \arrow[d,
      "\text{$[\metavar{m}{_3}[z] \mapsto \con{snd}(\metavar{m}{_6}[z])]$}"',
      "\text{\textbf{imitate axiom} ($\beta_{\pi_2}$)}"]
    \\
    \arrow[d,
      "\text{$[\metavar{m}{_6}[z] \mapsto z ]$}"',
      "\text{\textbf{project}}"]
    \\
    \arrow[d,
      "\metasubst{\mathsf{id}}"',
      "\text{\textbf{mutate} via $ \con{snd}(\con{pair}(\metavar{m}{_7}[g,y], \metavar{m}{_8}[g,y])) \equiv \metavar{m}{_8}[g,y] $ }"]
    \\
    \arrow[d,
      "\metasubst{\mathsf{id}}"',
      "\text{\textbf{decompose}}"]
    \\
    \arrow[d,
      "\text{$[\metavar{m}{_8}[g,y] \mapsto \con{abs}(x. \metavar{m}{_5}[x,g,y]) ]$}"',
      "\text{\textbf{eliminate*}}"]
    \\
    \arrow[d,
      "\metasubst{\mathsf{id}}"',
      "\text{\textbf{decompose} ($\con{pair}$)}"]
    \\
    \arrow[d,
      "\text{$[\metavar{m}{_7}[g,y] \mapsto g ]$}"',
      "\text{\textbf{eliminate*}}"]
    \\
    \arrow[d,
      "\metasubst{\mathsf{id}}"',
      "\text{\textbf{decompose} ($\con{abs}$)}"]
    \\
    \arrow[d,
      "\text{$[\metavar{m}{_5}[x,g,y] \mapsto \con{app}(x,y) ]$}"',
      "\text{\textbf{eliminate*}}"]
    \\
    \arrow[d,
      "\text{$[\metavar{m}{_5}[x,g,y] \mapsto \con{app}(x,y) ]$}"',
      "\text{\textbf{eliminate*}}"]
    \\
    \{
      \highlight{\con{app}(\metavar{m}{_4}[\con{pair}(g, \con{abs}(h.\con{app}(h, y)))], y) \meq \con{app}(g, y)}
    \}
    \arrow[d,
      "\metasubst{\mathsf{id}}"',
      "\text{\textbf{decompose} ($\con{app}$)}"]
    \\
    \arrow[d,
      "\metasubst{\mathsf{id}}"',
      "\text{\textbf{delete} ($\forall g,y. y \meq y$)}"]
    \\
    \arrow[d,
      "\text{$[\metavar{m}{_4}[z] \mapsto \con{fst}(\metavar{m}{_9}[z])]$}"',
      "\text{\textbf{imitate axiom} ($\beta_{\pi_1}$)}"]
    \\
    \arrow[d,
      "\text{$[\metavar{m}{_9}[z] \mapsto z ]$}"',
      "\text{\textbf{project}}"]
    \\
    \arrow[d,
      "\metasubst{\mathsf{id}}"',
      "\text{\textbf{mutate} via $ \con{fst}(\con{pair}(\metavar{m}{_{10}}[g,y], \metavar{m}{_{11}}[g,y])) \equiv \metavar{m}{_{10}}[g,y] $ }"]
    \\
    \arrow[d,
      "\metasubst{\mathsf{id}}"',
      "\text{\textbf{decompose}}"]
    \\
    \arrow[d,
      "\text{$[\metavar{m}{_{10}}[g,y] \mapsto g ]$}"',
      "\text{\textbf{eliminate*}}"]
    \\
    \arrow[d,
      "\metasubst{\mathsf{id}}"',
      "\text{\textbf{decompose} ($\con{pair}$)}"]
    \\
    \arrow[d,
      "\metasubst{\mathsf{id}}"',
      "\text{\textbf{delete} ($\forall g, y. g \meq g$)}"]
    \\
    \arrow[d,
      "\text{$[\metavar{m}{_{11}}[g,y] \mapsto \con{abs}(h.\con{app}(h, y)) ]$}"',
      "\text{\textbf{eliminate*}}"]
    \\
    \varnothing
   \end{tikzcd}

  \end{mdframed}
  \caption{Sample search path, exhibiting many rules, for an $E$-unification problem in $\lambda$-calculus: $\exists \m : \type{((\sigma \Rightarrow \tau) \times \sigma) \Rightarrow \tau}. \; \forall g : \type{\sigma \Rightarrow \tau}, y : \type{\sigma}. \; \m \; \langle g, \lambda h. h \; y \rangle \meq g \; y : \type{\tau}$. Types are omitted to save space. Composition of substitutions yields $[\m[] \mapsto \con{abs}(x. \con{app}(\con{snd}(x), \con{fst}(x))), \ldots ]$.}
  \label{figure:procedure-example}
\end{figure}


==> figures/unification-procedure.tex <==
\begin{figure*}
  \begin{mdframed}
  \begin{prooftree}
    \AxiomC{}
    \RightLabel{delete}
    \UnaryInfC{$
      \langle \{ \forall \Gamma . \color{blue}t \meq t\color{black} : \tau \} \cup S , \theta \rangle
    \longrightarrow \langle S, \theta \rangle
  $}
  \end{prooftree}

  \begin{prooftree}
    \AxiomC{$t_i \equiv x_i$ for all $i \in \{1, \ldots, k\}$}
    \noLine
    \UnaryInfC{$x_1, \ldots, x_k$ are distinct variables in $\Gamma$}
    \noLine
    \UnaryInfC{$\m$ does not occur in $u$
      \quad\quad
    $FV(u) \subseteq \{ x_1, \ldots, x_k \}$}
    \RightLabel{eliminate}
    \UnaryInfC{$
      \langle \{ \forall \Gamma . \color{blue}\m[t_1, \ldots, t_k] \meq u\color{black} : \tau \} \cup S
    , \theta
  \rangle 
    \longrightarrow \langle \{ S, \color{red}[\m[x_1, \ldots, x_k] \mapsto u]\color{black} \circ \theta \rangle
  $}
  \end{prooftree}

  \begin{prooftree}
    \AxiomC{$\defcon : (\overline{\sigma_1}.\tau_1, \ldots, \overline{\sigma_n}.\tau_n) \to \tau$}
    \RightLabel{decompose}
    \UnaryInfC{$
      \langle \{ \forall \Gamma . \color{blue}\defcon(\overline{x_1}.t_1, \ldots, \overline{x_n}.t_n) \meq \defcon(\overline{x_1}.u_1, \ldots, \overline{x_n}.u_n)\color{black} : \tau \} \cup S
    , \theta
  \rangle $}
  \noLine
  \UnaryInfC{$
    \longrightarrow \langle \{
      \forall \Gamma, \overline{x_i} : \overline{\sigma_i} . \color{blue}t_i \meq u_i\color{black} : \tau_i
    \}^{i \in \{1, \ldots, n\}}
    \cup S, \theta \rangle
  $}
  \end{prooftree}

  \begin{prooftree}
    \AxiomC{$\defcon : (\overline{\sigma_1}.\tau_1, \ldots, \overline{\sigma_n}.\tau_n) \to \tau$}
    \noLine
    \UnaryInfC{$(\Theta \mid \cdot \vdash \color{orange}o(\overline{x_1}.l_1, \ldots, \overline{x_n}.l_n) = r : \tau\color{black}) \in E$}
    \RightLabel{mutate (operator)}
    \UnaryInfC{$
      \langle \{ \forall \Gamma . \color{blue}\defcon(\overline{x_1}.t_1, \ldots, \overline{x_n}.t_n) \meq u \color{black} : \tau \} \cup S
    , \theta
  \rangle$}
  \noLine
  \UnaryInfC{$
    \longrightarrow \langle \{
      \forall \Gamma, \overline{x_i} : \overline{\sigma_i} . \color{blue}t_i \meq l_i \color{black} : \tau_i
    \}^{i \in \{1, \ldots, n\}}
    \cup \{ \Gamma : \overline{\sigma_n} . \color{blue} r \meq u \color{black} : \tau \}
    \cup S, \theta \rangle
  $}
  \end{prooftree}

  \begin{prooftree}
    \AxiomC{$\defcon : (\overline{\sigma_1}.\tau_1, \ldots, \overline{\sigma_n}.\tau_n) \to \tau$}
    \noLine
    \UnaryInfC{$(\Theta \mid \cdot \vdash \color{orange}o(\overline{x_1}.l_1, \ldots, \overline{x_n}.l_n) = r : \tau\color{black}) \in E$}
    \noLine
    \UnaryInfC{
    $(\m : [\rho_1, \ldots, \rho_k]\tau) \in \Theta$}
    \noLine
    \UnaryInfC{
    $\m_i : [\rho_1, \ldots, \rho_k, \overline{\sigma_i}]\tau_i$
    is fresh for all $i \in \{1, \ldots, n\}$}
    \RightLabel{mutate (meta)}
    \UnaryInfC{$
      \langle \{ \forall \Gamma . \color{blue}\m[t_1, \ldots, t_k] \meq u \color{black} : \tau \} \cup S
    , \theta
  \rangle$}
  \noLine
  \UnaryInfC{$
    \longrightarrow \langle
    \{ \forall \Gamma, \overline{x_i} : \overline{\sigma_i} . \color{blue}\m_i[t_1, \ldots, t_k, \overline{x_i}] \meq l_i \color{black} : \tau_i
    \}^{i \in \{1, \ldots, n\}}
    \cup \{ \Gamma : \overline{\sigma_n} . \color{blue} r \meq u \color{black} : \tau \}
  \cup S, $}
  \noLine
  \UnaryInfC{$\color{red}
    [\m[\overline{z}] \mapsto \defcon(\overline{x_1}.\metavar{\m}{1}[\overline{z}, \overline{x_1}], \ldots, \overline{x_n}.\metavar{\m}{n}[\overline{z}, \overline{x_n}]]
    \color{black}
    \circ \theta \rangle
  $}
  \end{prooftree}

  \begin{prooftree}
    \AxiomC{$\defcon : (\overline{\sigma_1}.\tau_1, \ldots, \overline{\sigma_n}.\tau_n) \to \tau$}
    \noLine
    \UnaryInfC{$(\m : [\rho_1, \ldots, \rho_k]\tau) \in \Theta$\quad\quad\quad
    $\m$ does not occur in $u_1, \ldots, u_n$}
    \noLine
    \UnaryInfC{
    $\m_i : [\rho_1, \ldots, \rho_k, \overline{\sigma_i}]\tau_i$
    is fresh for all $i \in \{1, \ldots, n\}$}
    \RightLabel{imitate}
    \UnaryInfC{$
      \langle \{ \forall \Gamma . \color{blue}\m[t_1, \ldots, t_k] \meq \defcon(\overline{x_1}.u_1, \ldots, \overline{x_n}.u_n) \color{black} : \tau \} \cup S
    , \theta
  \rangle $}
  \noLine
  \UnaryInfC{$
    \longrightarrow \langle
    \{ \forall \Gamma, \overline{x_i} : \overline{\sigma_i} . \color{blue}\m_i[t_1, \ldots, t_k, \overline{x_i}] \meq u_i \color{black} : \tau_i
    \}^{i \in \{1, \ldots, n\}}
  \cup S, $}
  \noLine
  \UnaryInfC{$\color{red}
    [\m[\overline{z}] \mapsto \defcon(\overline{x_1}.\metavar{\m}{1}[\overline{z}, \overline{x_1}], \ldots, \overline{x_n}.\metavar{\m}{n}[\overline{z}, \overline{x_n}]]
    \color{black}
    \circ \theta \rangle
  $}
  \end{prooftree}

  \begin{prooftree}
    \AxiomC{$(\m : [\rho_1, \ldots, \rho_k]\tau) \in \Theta$}
    \AxiomC{$\m$ does not occur in $u$}
    \AxiomC{$i \in \{1, \ldots, k\}$}
    \RightLabel{project$_i$}
    \TrinaryInfC{$
      \langle \{ \forall \Gamma . \color{blue}\m[t_1, \ldots, t_k] \meq u \color{black} : \tau \} \cup S
    , \theta
  \rangle $}
  \noLine
  \UnaryInfC{$
    \quad\quad\quad\quad
    \longrightarrow \langle
    \{ \forall \Gamma . \color{blue}t_i \meq u \color{black} : \tau \}
  \cup S,
    \color{red}
    [\m[\overline{z}] \mapsto z_i]
    \color{black}
    \circ \theta \rangle
  $}
  \end{prooftree}
  \end{mdframed}

  \caption{Unification rules in an ambient context $\Theta \mid \cdot$ over a second-order signature $\Sigma$.}
  \label{figure:unification-procedure}
\end{figure*}


==> sections/A-notation.tex <==
\section{Notation}

This is a summary of notation used in this paper:

\begin{itemize}
  \item Lowercase letters $x, y, z$ denote variables;
  \item Small capital letters $\m, \metavar{F}{}, \metavar{G}{}$ denote metavariables;
  \item Names in sans-serif font $\defcon, \con{op}, \con{app}, \con{mu}$ denote operators;
  \item Capital Greek letter $\Sigma$ denotes a signature;
  %\item Capital letter $E$ denotes a set of equalities;
  \item Capital Greek letters $\Theta, \Xi$ denote metavariable contexts;
  \item Capital Greek letters $\Gamma, \Delta$ denote variable contexts;
  \item Lowercase Greek letters $\type{\alpha}, \type{\beta}, \type{\sigma}, \type{\tau}$ denote types;
  \item Lowercase Greek letters $\metasubst{\eta}, \metasubst{\zeta}, \metasubst{\theta}, \metasubst{\xi}$ denote (meta)substitutions.
\end{itemize}

